Gait Events Prediction using Hybrid CNN-RNN-based Deep Learning models through a Single Waist-worn Wearable Sensor

Elderly gait is a source of rich information about their physical and mental health condition. As an alternative to the multiple sensors on the lower body parts, a single sensor on the pelvis has a positional advantage and an abundance of information acquirable. This study aimed to explore a way of improving the accuracy of gait event detection in the elderly using a single sensor on the waist and deep learning models. Data was gathered from elderly subjects equipped with three IMU sensors while they walked. The input was taken only from the waist sensor was used to train 16 deep-learning models including CNN, RNN, and CNN-RNN hybrid with or without the Bidirectional and Attention mechanism. The groundtruth was extracted from foot IMU sensors. Fairly high accuracy of 99.73% and 93.89% was achieved by the CNN-BiGRU-Att model at the tolerance window of $\pm$6TS ($\pm$6ms) and $\pm$1TS ($\pm$1ms) respectively. Advancing from the previous studies exploring gait event detection, the model showed a great improvement in terms of its prediction error having an MAE of 6.239ms and 5.24ms for HS and TO events respectively at the tolerance window of $\pm$1TS. The results showed that the use of CNN-RNN hybrid models with Attention and Bidirectional mechanisms is promising for accurate gait event detection using a single waist sensor. The study can contribute to reducing the burden of gait detection and increase its applicability in future wearable devices that can be used for remote health monitoring (RHM) or diagnosis based thereon.

==> bib_2.bib.tex <==
@techreport{nations2020world,
  author        = "Department of Economic and Social Affairs",
  title         = "World population ageing 2020: Highlights",
  institution   = "United Nations",
  year          = "2020"
}

@article{majumder2017wearable,
  title={Wearable sensors for remote health monitoring},
  author={Majumder, Sumit and Mondal, Tapas and Deen, M Jamal},
  journal={Sensors},
  volume={17},
  number={1},
  pages={130},
  year={2017},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{arshad2021gait,
  title={Gait-based Frailty Assessment using Image Representation of IMU Signals and Deep CNN},
  author={Arshad, Muhammad Zeeshan and Jung, Dawoon and Park, Mina and Shin, Hyungeun and Kim, Jinwook and Mun, Kyung-Ryoul},
  booktitle={2021 43rd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
  pages={1874--1879},
  year={2021},
  organization={IEEE}
}

@article{verghese2008gait,
  title={Gait dysfunction in mild cognitive impairment syndromes},
  author={Verghese, Joe and Robbins, Matthew and Holtzer, Roee and Zimmerman, Molly and Wang, Cuiling and Xue, Xiaonan and Lipton, Richard B},
  journal={Journal of the American Geriatrics Society},
  volume={56},
  number={7},
  pages={1244--1251},
  year={2008},
  publisher={Wiley Online Library}
}

@article{hannink2016sensor,
  title={Sensor-based gait parameter extraction with deep convolutional neural networks},
  author={Hannink, Julius and Kautz, Thomas and Pasluosta, Cristian F and Ga{\ss}mann, Karl-G{\"u}nter and Klucken, Jochen and Eskofier, Bjoern M},
  journal={IEEE journal of biomedical and health informatics},
  volume={21},
  number={1},
  pages={85--93},
  year={2016},
  publisher={IEEE}
}

@article{soaz2015step,
  title={Step detection and parameterization for gait assessment using a single waist-worn accelerometer},
  author={Soaz, Cristina and Diepold, Klaus},
  journal={IEEE Transactions on Biomedical Engineering},
  volume={63},
  number={5},
  pages={933--942},
  year={2015},
  publisher={IEEE}
}

@article{mccamley2012enhanced,
  title={An enhanced estimate of initial contact and final contact instants of time using lower trunk inertial sensor data},
  author={McCamley, John and Donati, Marco and Grimpampi, Eleni and Mazza, Claudia},
  journal={Gait \& posture},
  volume={36},
  number={2},
  pages={316--318},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{yang2019machine,
  title={Machine learning based adaptive gait phase estimation using inertial measurement sensors},
  author={Yang, Jianfu and Huang, Tzu-Hao and Yu, Shuangyue and Yang, Xiaolong and Su, Hao and Spungen, Ann M and Tsai, Chung-Ying},
  booktitle={Frontiers in Biomedical Devices},
  volume={41037},
  pages={V001T09A010},
  year={2019},
  organization={American Society of Mechanical Engineers}
}

@article{iijima2020state,
  title={State of the Field of waist-mounted sensor algorithm for gait events detection: A scoping review},
  author={Iijima, Hirotaka and Takahashi, Masaki},
  journal={Gait \& posture},
  volume={79},
  pages={152--161},
  year={2020},
  publisher={Elsevier}
}

@article{gonzalez2010real,
  title={Real-time gait event detection for normal subjects from lower trunk accelerations},
  author={Gonz{\'a}lez, Rafael C and L{\'o}pez, Antonio M and Rodriguez-Ur{\'\i}a, Javier and Alvarez, Diego and Alvarez, Juan C},
  journal={Gait \& posture},
  volume={31},
  number={3},
  pages={322--325},
  year={2010},
  publisher={Elsevier}
}

@article{nazarahari2021foot,
  title={Foot angular kinematics measured with inertial measurement units: A reliable criterion for real-time gait event detection},
  author={Nazarahari, Milad and Khandan, Aminreza and Khan, Atif and Rouhani, Hossein},
  journal={Journal of Biomechanics},
  pages={110880},
  year={2021},
  publisher={Elsevier}
}

@article{bloem1992investigation,
  title={Investigation of gait in elderly subjects over 88 years of age},
  author={Bloem, Bastiaan R and Haan, Joost and Lagaay, Anne M and van Beek, Wim and Wintzen, Axel R and Roos, Raymund AC},
  journal={Topics in geriatrics},
  volume={5},
  number={2},
  pages={78--84},
  year={1992},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{studenski2011gait,
  title={Gait speed and survival in older adults},
  author={Studenski, Stephanie and Perera, Subashan and Patel, Kushang and Rosano, Caterina and Faulkner, Kimberly and Inzitari, Marco and Brach, Jennifer and Chandler, Julie and Cawthon, Peggy and Connor, Elizabeth Barrett and others},
  journal={Jama},
  volume={305},
  number={1},
  pages={50--58},
  year={2011},
  publisher={American Medical Association}
}


@article{bloem1992investigation,
  title={Investigation of gait in elderly subjects over 88 years of age},
  author={Bloem, Bastiaan R and Haan, Joost and Lagaay, Anne M and van Beek, Wim and Wintzen, Axel R and Roos, Raymund AC},
  journal={Topics in geriatrics},
  volume={5},
  number={2},
  pages={78--84},
  year={1992},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{studenski2011gait,
  title={Gait speed and survival in older adults},
  author={Studenski, Stephanie and Perera, Subashan and Patel, Kushang and Rosano, Caterina and Faulkner, Kimberly and Inzitari, Marco and Brach, Jennifer and Chandler, Julie and Cawthon, Peggy and Connor, Elizabeth Barrett and others},
  journal={Jama},
  volume={305},
  number={1},
  pages={50--58},
  year={2011},
  publisher={American Medical Association}
}

@inproceedings{yu2021gait,
  title={Gait Phase Detection Based on a Foot-Mounted Inertial Sensor Using Long Short-Term Memory Enhanced by Hidden Markov Model},
  author={Yu, Zhipeng and Zhao, Jianghai and Zhou, Xiong and Liu, Kun and Yan, Yu},
  booktitle={2021 26th International Conference on Automation and Computing (ICAC)},
  pages={1--5},
  year={2021},
  organization={IEEE}
}

@article{figueiredo2018gait,
  title={Gait event detection in controlled and real-life situations: Repeated measures from healthy subjects},
  author={Figueiredo, Joana and Felix, Paulo and Costa, Luis and Moreno, Juan C and Santos, Cristina P},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={26},
  number={10},
  pages={1945--1956},
  year={2018},
  publisher={IEEE}
}

@book{whittle2014gait,
  title={Gait analysis: an introduction},
  author={Whittle, Michael W},
  year={2014},
  publisher={Butterworth-Heinemann}
}

@misc{arshad2021gaitbased,
      title={Gait-based Frailty Assessment using Image Representation of IMU Signals and Deep CNN}, 
      author={Muhammad Zeeshan Arshad and Dawoon Jung and Mina Park and Hyungeun Shin and Jinwook Kim and Kyung-Ryoul Mun},
      year={2021},
      eprint={2110.07821},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@ARTICLE{9383834,
  author={Jung, Dawoon and Kim, Jinwook and Kim, Miji and Won, Chang Won and Mun, Kyung-Ryoul},
  journal={IEEE Journal of Biomedical and Health Informatics}, 
  title={Frailty Assessment Using Temporal Gait Characteristics and a Long Short-Term Memory Network}, 
  year={2021},
  volume={25},
  number={9},
  pages={3649-3658},
  doi={10.1109/JBHI.2021.3067931}}

@article{jung2021classifying,
  title={Classifying the Risk of Cognitive Impairment Using Sequential Gait Characteristics and Long Short-Term Memory Networks},
  author={Jung, Dawoon and Kim, Jinwook and Kim, Miji and Won, Chang Won and Mun, Kyung-Ryoul},
  journal={IEEE Journal of Biomedical and Health Informatics},
  year={2021},
  publisher={IEEE}
}

@article{folstein1975mini,
  title={“Mini-mental state”: a practical method for grading the cognitive state of patients for the clinician},
  author={Folstein, Marshal F and Folstein, Susan E and McHugh, Paul R},
  journal={Journal of psychiatric research},
  volume={12},
  number={3},
  pages={189--198},
  year={1975},
  publisher={Pergamon}
}

@article{morley2012simple,
  title={A simple frailty questionnaire (FRAIL) predicts outcomes in middle aged African Americans},
  author={Morley, John E and Malmstrom, TK and Miller, DK},
  journal={The journal of nutrition, health \& aging},
  volume={16},
  number={7},
  pages={601--608},
  year={2012},
  publisher={Springer}
}

@article{taborri2014novel,
  title={A novel HMM distributed classifier for the detection of gait phases by means of a wearable inertial sensor network},
  author={Taborri, Juri and Rossi, Stefano and Palermo, Eduardo and Patan{\`e}, Fabrizio and Cappa, Paolo},
  journal={Sensors},
  volume={14},
  number={9},
  pages={16212--16234},
  year={2014},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{yuwono2014unsupervised,
  title={Unsupervised nonparametric method for gait analysis using a waist-worn inertial sensor},
  author={Yuwono, Mitchell and Su, Steven W and Guo, Ying and Moulton, Bruce D and Nguyen, Hung T},
  journal={Applied Soft Computing},
  volume={14},
  pages={72--80},
  year={2014},
  publisher={Elsevier}
}

@article{de2019concurrent,
  title={Concurrent validity of a commercial wireless trunk triaxial accelerometer system for gait analysis},
  author={De Ridder, Roel and Lebleu, Julien and Willems, Tine and De Blaiser, Cedric and Detrembleur, Christine and Roosen, Philip},
  journal={Journal of sport rehabilitation},
  volume={28},
  number={6},
  year={2019},
  publisher={Human Kinetics}
}

@article{pham2017validation,
  title={Validation of a step detection algorithm during straight walking and turning in patients with Parkinson’s disease and older adults using an inertial measurement unit at the lower back},
  author={Pham, Minh H and Elshehabi, Morad and Haertner, Linda and Del Din, Silvia and Srulijes, Karin and Heger, Tanja and Synofzik, Matthis and Hobert, Markus A and Faber, Gert S and Hansen, Clint and others},
  journal={Frontiers in neurology},
  volume={8},
  pages={457},
  year={2017},
  publisher={Frontiers}
}

@inproceedings{digo2021gait,
  title={Gait Phases Detection in Elderly using Trunk-MIMU System.},
  author={Digo, Elisa and Agostini, Valentina and Pastorelli, Stefano and Gastaldi, Laura and Panero, Elisa},
  booktitle={BIODEVICES},
  pages={58--65},
  year={2021}
}

@article{rantalainen2020gait,
  title={Gait variability using waist-and ankle-worn inertial measurement units in healthy older adults},
  author={Rantalainen, Timo and Karavirta, Laura and Pirkola, Henrikki and Rantanen, Taina and Linnamo, Vesa},
  journal={Sensors},
  volume={20},
  number={10},
  pages={2858},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{o2019augmenting,
  title={Augmenting clinical outcome measures of gait and balance with a single inertial sensor in age-ranged healthy adults},
  author={O’Brien, Megan K and Hidalgo-Araya, Marco D and Mummidisetty, Chaithanya K and Vallery, Heike and Ghaffari, Roozbeh and Rogers, John A and Lieber, Richard and Jayaraman, Arun},
  journal={Sensors},
  volume={19},
  number={20},
  pages={4537},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{gonccalves2018real,
  title={Real-time tool for human gait detection from lower trunk acceleration},
  author={Gon{\c{c}}alves, Helena R and Moreira, Rui and Rodrigues, Ana and Minas, Gra{\c{c}}a and Reis, Lu{\'\i}s Paulo and Santos, Cristina P},
  booktitle={World Conference on Information Systems and Technologies},
  pages={9--18},
  year={2018},
  organization={Springer}
}

@article{zijlstra2003assessment,
  title={Assessment of spatio-temporal gait parameters from trunk accelerations during human walking},
  author={Zijlstra, Wiebren and Hof, At L},
  journal={Gait \& posture},
  volume={18},
  number={2},
  pages={1--10},
  year={2003},
  publisher={Elsevier}
}

@article{gonzalez2010real,
  title={Real-time gait event detection for normal subjects from lower trunk accelerations},
  author={Gonz{\'a}lez, Rafael C and L{\'o}pez, Antonio M and Rodriguez-Ur{\'\i}a, Javier and Alvarez, Diego and Alvarez, Juan C},
  journal={Gait \& posture},
  volume={31},
  number={3},
  pages={322--325},
  year={2010},
  publisher={Elsevier}
}

@article{sarshar2021gait,
  title={Gait phase estimation by using LSTM in IMU-based gait analysis—Proof of concept},
  author={Sarshar, Mustafa and Polturi, Sasanka and Schega, Lutz},
  journal={Sensors},
  volume={21},
  number={17},
  pages={5749},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{romijnders2021validation,
  title={Validation of IMU-based gait event detection during curved walking and turning in older adults and Parkinson’s Disease patients},
  author={Romijnders, Robbin and Warmerdam, Elke and Hansen, Clint and Welzel, Julius and Schmidt, Gerhard and Maetzler, Walter},
  journal={Journal of neuroengineering and rehabilitation},
  volume={18},
  number={1},
  pages={1--10},
  year={2021},
  publisher={Springer}
}

@article{fadillioglu2020automated,
  title={Automated gait event detection for a variety of locomotion tasks using a novel gyroscope-based algorithm},
  author={Fadillioglu, Cagla and Stetter, Bernd J and Ringhof, Steffen and Krafft, Frieder C and Sell, Stefan and Stein, Thorsten},
  journal={Gait \& Posture},
  volume={81},
  pages={102--108},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{lin2021gait,
  title={Gait Parameters Analysis Based on Leg-and-shoe-mounted IMU and Deep Learning},
  author={Lin, Po-Hsin and Shih, Chang-Lin and Wong, Davy PY and Chou, Pai H},
  booktitle={2021 International Symposium on VLSI Design, Automation and Test (VLSI-DAT)},
  pages={1--4},
  year={2021},
  organization={IEEE}
}

@article{bae2011gait,
  title={Gait phase analysis based on a Hidden Markov Model},
  author={Bae, Joonbum and Tomizuka, Masayoshi},
  journal={Mechatronics},
  volume={21},
  number={6},
  pages={961--970},
  year={2011},
  publisher={Elsevier}
}

@article{mannini2012gait,
  title={Gait phase detection and discrimination between walking--jogging activities using hidden Markov models applied to foot motion data from a gyroscope},
  author={Mannini, Andrea and Sabatini, Angelo Maria},
  journal={Gait \& posture},
  volume={36},
  number={4},
  pages={657--661},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{lee2009novel,
  title={Novel algorithm for the hemiplegic gait evaluation using a single 3-axis accelerometer},
  author={Lee, Hyo-Ki and Hwang, Sung-Jae and Cho, Sung-Pil and Lee, Dong-Ryul and You, Sung-Hyun and Lee, Kyoung-Joung and Kim, Yong-Ho and Choi, Ho-Seon},
  booktitle={2009 Annual International Conference of the IEEE Engineering in Medicine and Biology Society},
  pages={3964--3966},
  year={2009},
  organization={IEEE}
}

@article{mundt2020estimation,
  title={Estimation of gait mechanics based on simulated and measured IMU data using an artificial neural network},
  author={Mundt, Marion and Koeppe, Arnd and David, Sina and Witter, Tom and Bamer, Franz and Potthast, Wolfgang and Markert, Bernd},
  journal={Frontiers in bioengineering and biotechnology},
  volume={8},
  pages={41},
  year={2020},
  publisher={Frontiers}
}

@article{mielke2013assessing,
  title={Assessing the temporal relationship between cognition and gait: slow gait predicts cognitive decline in the Mayo Clinic Study of Aging},
  author={Mielke, Michelle M and Roberts, Rosebud O and Savica, Rodolfo and Cha, Ruth and Drubach, Dina I and Christianson, Teresa and Pankratz, Vernon S and Geda, Yonas E and Machulda, Mary M and Ivnik, Robert J and others},
  journal={Journals of Gerontology Series A: Biomedical Sciences and Medical Sciences},
  volume={68},
  number={8},
  pages={929--937},
  year={2013},
  publisher={Oxford University Press US}
}

@article{mannini2016machine,
  title={A machine learning framework for gait classification using inertial sensors: Application to elderly, post-stroke and huntington’s disease patients},
  author={Mannini, Andrea and Trojaniello, Diana and Cereatti, Andrea and Sabatini, Angelo M},
  journal={Sensors},
  volume={16},
  number={1},
  pages={134},
  year={2016},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{kim2017development,
  title={Development of an IMU-based foot-ground contact detection (FGCD) algorithm},
  author={Kim, Myeongkyu and Lee, Donghun},
  journal={Ergonomics},
  volume={60},
  number={3},
  pages={384--403},
  year={2017},
  publisher={Taylor \& Francis}
}

@article{zhen2019walking,
  title={Walking gait phase detection based on acceleration signals using LSTM-DNN Algorithm},
  author={Zhen, Tao and Yan, Lei and Yuan, Peng},
  journal={Algorithms},
  volume={12},
  number={12},
  pages={253},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{oudre2018template,
  title={Template-based step detection with inertial measurement units},
  author={Oudre, Laurent and Barrois-M{\"u}ller, R{\'e}mi and Moreau, Thomas and Truong, Charles and Vienne-Jumeau, Ali{\'e}nor and Ricard, Damien and Vayatis, Nicolas and Vidal, Pierre-Paul},
  journal={Sensors},
  volume={18},
  number={11},
  pages={4033},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{inman1953major,
  title={The major determinants in normal and pathological gait},
  author={Inman, Verne T and Eberhart, Howard D and others},
  journal={JBJS},
  volume={35},
  number={3},
  pages={543--558},
  year={1953},
  publisher={LWW}
}

@article{li20163d,
  title={3D tracking via shoe sensing},
  author={Li, Fangmin and Liu, Guo and Liu, Jian and Chen, Xiaochuang and Ma, Xiaolin},
  journal={Sensors},
  volume={16},
  number={11},
  pages={1809},
  year={2016},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{jasiewicz2006gait,
  title={Gait event detection using linear accelerometers or angular velocity transducers in able-bodied and spinal-cord injured individuals},
  author={Jasiewicz, Jan M and Allum, John HJ and Middleton, James W and Barriskill, Andrew and Condie, Peter and Purcell, Brendan and Li, Raymond Che Tin},
  journal={Gait \& posture},
  volume={24},
  number={4},
  pages={502--509},
  year={2006},
  publisher={Elsevier}
}

@article{perry2010gait,
  title={Gait analysis. Normal and pathological function 2nd ed},
  author={Perry, Jacquelin and Burnfield, Judith M},
  journal={California: Slack},
  year={2010}
}

@inproceedings{patterson2016validation,
  title={Validation of temporal gait metrics from three IMU locations to the gold standard force plate},
  author={Patterson, Matthew R and Johnston, William and O Mahony, Niamh and O Mahony, Sam and Nolan, Eimear and Caulfield, Brian},
  booktitle={2016 38th Annual International Conference of the IEEE Engineering in Medicine and Biology Society (EMBC)},
  pages={667--671},
  year={2016},
  organization={IEEE}
}

@article{taborri2014novel,
  title={A novel HMM distributed classifier for the detection of gait phases by means of a wearable inertial sensor network},
  author={Taborri, Juri and Rossi, Stefano and Palermo, Eduardo and Patan{\`e}, Fabrizio and Cappa, Paolo},
  journal={Sensors},
  volume={14},
  number={9},
  pages={16212--16234},
  year={2014},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{prasanth2021wearable,
  title={Wearable sensor-based real-time gait detection: a systematic review},
  author={Prasanth, Hari and Caban, Miroslav and Keller, Urs and Courtine, Gr{\'e}goire and Ijspeert, Auke and Vallery, Heike and Von Zitzewitz, Joachim},
  journal={Sensors},
  volume={21},
  number={8},
  pages={2727},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{o2019augmenting,
  title={Augmenting clinical outcome measures of gait and balance with a single inertial sensor in age-ranged healthy adults},
  author={O’Brien, Megan K and Hidalgo-Araya, Marco D and Mummidisetty, Chaithanya K and Vallery, Heike and Ghaffari, Roozbeh and Rogers, John A and Lieber, Richard and Jayaraman, Arun},
  journal={Sensors},
  volume={19},
  number={20},
  pages={4537},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{yuwono2014unsupervised,
  title={Unsupervised nonparametric method for gait analysis using a waist-worn inertial sensor},
  author={Yuwono, Mitchell and Su, Steven W and Guo, Ying and Moulton, Bruce D and Nguyen, Hung T},
  journal={Applied Soft Computing},
  volume={14},
  pages={72--80},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{gonccalves2018real,
  title={Real-time tool for human gait detection from lower trunk acceleration},
  author={Gon{\c{c}}alves, Helena R and Moreira, Rui and Rodrigues, Ana and Minas, Gra{\c{c}}a and Reis, Lu{\'\i}s Paulo and Santos, Cristina P},
  booktitle={World Conference on Information Systems and Technologies},
  pages={9--18},
  year={2018},
  organization={Springer}
}

@article{yetisen2018wearables,
  title={Wearables in medicine},
  author={Yetisen, Ali K and Martinez-Hurtado, Juan Leonardo and {\"U}nal, Bar{\i}{\c{s}} and Khademhosseini, Ali and Butt, Haider},
  journal={Advanced Materials},
  volume={30},
  number={33},
  pages={1706910},
  year={2018},
  publisher={Wiley Online Library}
}

@article{mahlknecht2013prevalence,
  title={Prevalence and burden of gait disorders in elderly men and women aged 60--97 years: a population-based study},
  author={Mahlknecht, Philipp and Kiechl, Stefan and Bloem, Bastiaan R and Willeit, Johann and Scherfler, Christoph and Gasperi, Arno and Rungger, Gregorio and Poewe, Werner and Seppi, Klaus},
  journal={PLoS One},
  volume={8},
  number={7},
  pages={e69627},
  year={2013},
  publisher={Public Library of Science San Francisco, USA}
}

@article{krebs1985reliability,
  title={Reliability of observational kinematic gait analysis},
  author={Krebs, David E and Edelstein, Joan E and Fishman, Sidney},
  journal={Physical Therapy},
  volume={65},
  number={7},
  pages={1027--1033},
  year={1985},
  publisher={Oxford University Press}
}

@article{barker2006accuracy,
  title={Accuracy, reliability, and validity of a spatiotemporal gait analysis system},
  author={Barker, Susan and Craik, Rebecca and Freedman, William and Herrmann, Nira and Hillstrom, Howard},
  journal={Medical engineering \& physics},
  volume={28},
  number={5},
  pages={460--467},
  year={2006},
  publisher={Elsevier}
}

@book{winter2009biomechanics,
  title={Biomechanics and motor control of human movement},
  author={Winter, David A},
  year={2009},
  publisher={John Wiley \& Sons}
}

@article{tao2012gait,
  title={Gait analysis using wearable sensors},
  author={Tao, Weijun and Liu, Tao and Zheng, Rencheng and Feng, Hutian},
  journal={Sensors},
  volume={12},
  number={2},
  pages={2255--2283},
  year={2012},
  publisher={Molecular Diversity Preservation International}
}

@article{jasiewicz2006gait,
  title={Gait event detection using linear accelerometers or angular velocity transducers in able-bodied and spinal-cord injured individuals},
  author={Jasiewicz, Jan M and Allum, John HJ and Middleton, James W and Barriskill, Andrew and Condie, Peter and Purcell, Brendan and Li, Raymond Che Tin},
  journal={Gait \& posture},
  volume={24},
  number={4},
  pages={502--509},
  year={2006},
  publisher={Elsevier}
}

@article{sabatini2005assessment,
  title={Assessment of walking features from foot inertial sensing},
  author={Sabatini, Angelo M and Martelloni, Chiara and Scapellato, Sergio and Cavallo, Filippo},
  journal={IEEE Transactions on biomedical engineering},
  volume={52},
  number={3},
  pages={486--494},
  year={2005},
  publisher={IEEE}
}

@article{kitagawa2016estimation,
  title={Estimation of foot trajectory during human walking by a wearable inertial measurement unit mounted to the foot},
  author={Kitagawa, Naoki and Ogihara, Naomichi},
  journal={Gait \& posture},
  volume={45},
  pages={110--114},
  year={2016},
  publisher={Elsevier}
}




@article{jasiewicz2006gait,
  title={Gait event detection using linear accelerometers or angular velocity transducers in able-bodied and spinal-cord injured individuals},
  author={Jasiewicz, Jan M and Allum, John HJ and Middleton, James W and Barriskill, Andrew and Condie, Peter and Purcell, Brendan and Li, Raymond Che Tin},
  journal={Gait \& posture},
  volume={24},
  number={4},
  pages={502--509},
  year={2006},
  publisher={Elsevier}
}

@inproceedings{abadi2016tensorflow,
  title={Tensorflow: A system for large-scale machine learning},
  author={Abadi, Mart{\'\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and others},
  booktitle={12th $\{$USENIX$\}$ symposium on operating systems design and implementation ($\{$OSDI$\}$ 16)},
  pages={265--283},
  year={2016}
}

@incollection{graves2012supervised,
  title={Supervised sequence labelling},
  author={Graves, Alex},
  booktitle={Supervised sequence labelling with recurrent neural networks},
  pages={5--13},
  year={2012},
  publisher={Springer}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  pages={5998--6008},
  year={2017}
}
